X-Reset: Scaling Object-Centric Reinforcement Learning via Cross-Embodiment Resets

Reinforcement learning (RL) in simulation can train dexterous manipulation policies without robot demonstrations, but training a single generalist policy with task-agnostic rewards faces a severe exploration problem: approaching, grasping, and reorienting diverse objects with many degrees of freedom is difficult to discover from scratch. Prior works make exploration tractable with high-quality robot demonstrations, per-task reward shaping, or by restricting policies to narrow modes of behavior. We propose X-Reset, a framework that instead resolves exploration with human hand-object demonstrations. Rather than imitating or tracking retargeted human motion, X-Reset kinematically retargets hand-object states to noisy robot states, filters out states that are unstable in simulation, and samples the remainder as resets during RL training with general-purpose object-centric rewards. The resulting policy depends only on object state and goal, with demonstrations entering training through the reset distribution. We show that X-Reset trains generalist policies on 20 objects across three embodiments---a 22-DoF hand on two different arms and a parallel-jaw gripper---and resolves the exploration challenges of RL from scratch. X-Reset scales with the number of training objects, generalizes to unseen objects, can learn from imperfect hand-pose estimates, and transfers behaviors zero-shot from sim-to-real.

==> figures_icra/teaser_top.tex <==
% Non-float teaser, injected into the title block via \@IEEEaftertitletext in
% main.tex so it sits at the top of page 1 spanning both columns. (A real
% figure* issued after \maketitle is always deferred to page 2 by ieeeconf.)
\begin{center}
  \includegraphics[width=\textwidth]{figures_icra/output_teaser.pdf}
  \captionof{figure}{\textbf{Overview of \methodname.} We introduce \methodname, a simple recipe to pair generalist object-centric RL in simulation with kinematically retargeted human hand-object states as resets. Learning to approach, grasp, and reorient objects from scratch results in a challenging exploration problem, while \methodname\ directly exposes policies to high-value states from which exploration is easy. \rev{With a common reward formulation, we train generalist policies for diverse robot embodiments and demonstrate sim-to-real transfer.}}
  \label{fig:teaser}
\end{center}

